Reusing Convolutional Neural Network Models through Modularization and Composition

With the widespread success of deep learning technologies, many trained deep neural network (DNN) models are now publicly available. However, directly reusing the public DNN models for new tasks often fails due to mismatching functionality or performance. Inspired by the notion of modularization and composition in software reuse, we investigate the possibility of improving the reusability of DNN models in a more fine-grained manner. Specifically, we propose two modularization approaches named CNNSplitter and GradSplitter, which can decompose a trained convolutional neural network (CNN) model for $N$-class classification into $N$ small reusable modules. Each module recognizes one of the $N$ classes and contains a part of the convolution kernels of the trained CNN model. Then, the resulting modules can be reused to patch existing CNN models or build new CNN models through composition. The main difference between CNNSplitter and GradSplitter lies in their search methods: the former relies on a genetic algorithm to explore search space, while the latter utilizes a gradient-based search method. Our experiments with three representative CNNs on three widely-used public datasets demonstrate the effectiveness of the proposed approaches. Compared with CNNSplitter, GradSplitter incurs less accuracy loss, produces much smaller modules (19.88% fewer kernels), and achieves better results on patching weak models. In particular, experiments on GradSplitter show that (1) by patching weak models, the average improvement in terms of precision, recall, and F1-score is 17.13%, 4.95%, and 11.47%, respectively, and (2) for a new task, compared with the models trained from scratch, reusing modules achieves similar accuracy (the average loss of accuracy is only 2.46%) without a costly training process. Our approaches provide a viable solution to the rapid development and improvement of CNN models.

==> discussion.tex <==
\subsection{Impact of Major Parameters on \projectName}
This section discusses the impact of major parameters in \projectName.
As shown in Algorithm \ref{algo:decom}, the major parameters includes $lr_h$ (the learning rate for training heads), $lr_m$ (the learning rate for training masks), and $\alpha$ (the weight value for the weighted sum of losses). 
\qi{DOING...}

\subsection{Threats to Validity}
\textbf{External validity:} Threats to external validity relate to the generalizability of our results. 
Some CNN models have different structures and sizes compared to SimCNN, ResCNN, and InceCNN. 
The results might not be generalizable to these CNN models. 
\Blue{For instance, CNNSplitter's performance is subject to the exponential search space. There exists a trade-off between the efficiency and quality of modularization, which is controlled by the number of groups.}
Moreover, the results are not validated on other datasets for different tasks. 
However, SimCNN, ResCNN, and InceCNN are representative CNN models and their structures are widely used in various tasks. 
Many different CNN models can be seen as variants of SimCNN, ResCNN, and InceCNN. 
In addition, CIFAR-10, and SVHN are representative datasets and are widely used for evaluation in related researches~\cite{nnmodularity2022icse,feng2020deepgini}. In our future work, more experiments will be conducted on a variety of CNN models and datasets to alleviate this threat.

\textbf{Internal validity:} An internal threat comes from the choice of datasets for evaluation. To mitigate this threat, in this study we use the CIFAR-10 and SVHN datasets 
from Pytorch, which are well organized and widely used.

\textbf{Construct validity:} In this study, a threat relates to the suitability of our evaluation metrics. 
The accuracy and the number of retained convolution kernels are used as the metrics to evaluate modularization. 
Moreover, the accuracy, time overhead, and GPU memory overhead are used to evaluated the composed model.
These metrics have also been used in other related work~\cite{fse2020modularity,nnmodularity2022icse}.


==> motivation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.65\columnwidth]{figures/motivation_example.pdf}
    \caption{Examples of reusing modules: (1) building a higher-accuracy composed CNN model for the same task, and (2) building a new composed CNN model for a new task.}
    \label{fig:motivation_example}
    \vspace{-6pt}
\end{figure}

Applying modularization and composition to the development of CNN models has several benefits.
As shown in Figure \ref{fig:motivation_example}, there are two trained CNN models (\ie $\mathit{TM}_0$ and $\mathit{TM}_1$) for Task 1, which classify ``horse'', ``deer'', and ``dog''. There are also  two trained CNN models (\ie $TM_2$ and $TM_3$) for Task 2, which classify ``bird'' and ``cat''. 
We could decompose the trained CNN models into smaller modules and later reuse these modules. 
Each module corresponds to a class called the \textit{target class}. A module is a binary classifier and can recognize whether or not an input belongs to a target class.
For instance, $TM_0$ can be decomposed into 3 modules, each of which is a binary classification sub-model of $TM_0$.
The module $m_0^1$ can recognize whether an input image belongs to ``deer'', and its target class is ``deer''.

Based on the reusable modules:
(1) for the same task, such as Task 1, developers %
can evaluate the modules of $TM_0$ and $TM_1$ on the corresponding binary classification tasks using their own testing data. 
Then, developers can reuse the modules with the best performance in binary classification to build a \textit{CM} (composed model).
In this example, $m_1^0$, $m_0^1$, and $m_1^2$ have the best performance in classifying ``horse'', ``deer'', and ``dog'', respectively. 
As a result, the \textit{CM} is built by reusing $m_1^0$, $m_0^1$, and $m_1^2$ and can outperform both $TM_0$ and $TM_1$.
(2) for a new task, such as Task 3 that classifies ``dog'' and ``cat'', developers can evaluate the four modules
which recognize ``dog'' and ``cat''. 
Based on the evaluation results, $m_1^2$ and $m_2^1$ are reused to build a \textit{CM}.
Compared with the model trained for Task 3 from scratch, the \textit{CM} can achieve competitive performance without costly training.

\begin{figure}[t]
	\centering
	\includegraphics[width=8.8cm]{figures/module.pdf}
    \caption{An illustration of creating a module through $mask \odot TM \oplus head$.}
    \label{fig:module}
    \vspace{-6pt}
\end{figure}

To achieve the modularization of a \textit{TM}, a \textit{mask} and a \textit{head} are used to create a module through $mask \odot TM \oplus head$. 
Figure \ref{fig:module} illustrates the creation of a module.
A \textit{mask} consists of an array of 0s and 1s, where 0 (or 1) indicates that the corresponding convolution kernels in the \textit{TM} are removed (or retained). 
The operation $mask \odot TM$ removes kernels from \textit{TM}, resulting in a \textit{masked TM}.
A \textit{head} consists of FC layers and converts an $N$-dimensional input into a $1$-dimensional output.
The operation $\oplus head$ appends a \textit{head} after the \textit{masked TM}, resulting in a module. 
As a result, the constructed module is a binary classifier. 
The output value of a module greater than 0.5 indicates that the input belongs to the target class, and vice versa.

Based on the above module creation, the decomposition of an $N$-class \textit{TM} is a training process that jointly optimizes $N$ masks and $N$ heads on the $N$-class classification task.
During the forward propagation, $N$ modules run separately. The outputs of $N$ modules are concatenated into an $N$-dimensional vector, which is the prediction of $N$-class classification.
The loss consists of (1) the cross-entropy between the prediction and the actual label and (2) the percentage of retained kernels in $N$ modules.
For the backward propagation, a gradient descent-based optimization is used to minimize the loss.
As a result, each module retains a part of convolution kernels while keeping sufficient ability to recognize the target class.

